Optimizing Huffman Decoding for Error-Bounded Lossy Compression on GPUs

More and more HPC applications require fast and effective compression techniques to handle large volumes of data in storage and transmission. Not only do these applications need to compress the data effectively during simulation, but they also need to perform decompression efficiently for post hoc analysis. SZ is an error-bounded lossy compressor for scientific data, and cuSZ is a version of SZ designed to take advantage of the GPU's power. At present, cuSZ's compression performance has been optimized significantly while its decompression still suffers considerably lower performance because of its sophisticated lossless compression step -- a customized Huffman decoding. In this work, we aim to significantly improve the Huffman decoding performance for cuSZ, thus improving the overall decompression performance in turn. To this end, we first investigate two state-of-the-art GPU Huffman decoders in depth. Then, we propose a deep architectural optimization for both algorithms. Specifically, we take full advantage of CUDA GPU architectures by using shared memory on decoding/writing phases, online tuning the amount of shared memory to use, improving memory access patterns, and reducing warp divergence. Finally, we evaluate our optimized decoders on an Nvidia V100 GPU using eight representative scientific datasets. Our new decoding solution obtains an average speedup of 3.64X over cuSZ's Huffman decoder and improves its overall decompression performance by 2.43X on average.

==> listing2/eval-cusz.tex <==
	cuSZ baseline	Opt. Self Sync	Opt. Gap Array
HACC	44.5	106.1269623	127.6274849
EXAALT	43.6	92.43032214	117.2804186
CESM-ATM	42.9	117.1970179	130.4722814
Nyx	78.4	108.6767519	127.2653227
ISABEL	41.7	97.94889434	110.4804501


==> listing2/self-sync.tex <==
\footnotesize\centering\ttfamily
\begin{tabular}{@{} >{\bfseries\ttfamily}rr @{}}
Symbol & Codeword \\
\cmidrule[.5pt](lr){1-2}
\end{tabular}

==> setting/_metadata.tex <==

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%\begin{CCSXML}
%<ccs2012>
%   <concept>
%       <concept_id>10003752.10003809.10010170.10010174</concept_id>
%       <concept_desc>Theory of computation~Massively parallel algorithms</concept_desc>
%       <concept_significance>500</concept_significance>
%       </concept>
% </ccs2012>
%\end{CCSXML}

%\ccsdesc[500]{Theory of computation~Massively parallel algorithms}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.

%\keywords{GPU, Massively Parallel, Lossy Compression}

%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

==> setting/acm_template_setting.tex <==

%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
% \setcopyright{acmcopyright}
% \copyrightyear{2018}
% \acmYear{2018}
% \acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
% \acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
% \acmConference[ICS '20]{PPoPP '21: ACM International Conference on Supercomputing}{June 29--July 02, 2020}{Barcelona, Spain}
\acmConference[PPoPP '21]{Principles and Practice of Parallel Programming}{February 27--March 3, 2021}{Seoul, South Korea}
% \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection, June 03--05, 2018, Woodstock, NY}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

%%
%% end of the preamble, start of the body of the document source.


%% \title moved to text
%% \title[short title]{full title}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.


\author{Jiannan Tian}
\affiliation{%
	\institution{Washington State University}
	\city{Pullman}\state{WA}\country{USA}
}
\email{jiannan.tian@wsu.edu}


\author{Cody Rivera}
\affiliation{%
	\institution{The University of Alabama}
	\city{Tuscaloosa}\state{AL}\country{USA}
}
\email{cjrivera1@crimson.ua.edu}


\author{Jieyang Chen}
\affiliation{%
	\institution{Oak Ridge National Laboratory}
	\city{Oak Ridge}\state{TN}\country{USA}
}
\email{chenj3@ornl.gov}


\author{Sheng Di}
\affiliation{%
	\institution{Argonne National Laboratory}
	\city{Lemont}\state{IL}\country{USA}
}
\email{sdi1@anl.gov}


\author{Dingwen Tao}
\authornote{Corresponding author: Dingwen Tao, School of EECS, Washington State University, Pullman, WA 99164, USA.}
\affiliation{%
	\institution{Washington State University}
	\city{Pullman}\state{WA}\country{USA}
}
\email{dingwen.tao@wsu.edu}


\author{Franck Cappello}
\affiliation{%
	\institution{Argonne National Laboratory}
	\city{Lemont}\state{IL}\country{USA}
}
\email{cappello@mcs.anl.gov}

\renewcommand{\shortauthors}{Tian et~al.}

\settopmatter{printacmref=false}
\setcopyright{none}
\renewcommand\footnotetextcopyrightpermission[1]{}
\pagestyle{plain}

==> tikz2/_tikz_preamble_nodocclass.tex <==

\usepackage[utf8]{inputenc}

\usepackage{textcomp} 
\usepackage{textgreek}

\usepackage[usenames]{color} 

%used for font color
\usepackage{amssymb, amsmath, bm} 
%\usepackage{sfmath}

%useful to type directly diacritic characters
\usepackage{tikz} 
\usetikzlibrary{shadings} 
\usetikzlibrary{positioning}
\usetikzlibrary{graphs}
\usepackage{booktabs}

% \usepackage[margin=.75in, bottom=1in]{geometry}
\usepackage{lipsum}

\usepackage{xcolor}

\usetikzlibrary{shadows.blur}

\definecolor{RED}{HTML}{d7003a} 
\definecolor{BLUE}{HTML}{003399}
\definecolor{BLUE2}{HTML}{2B66D3}
\definecolor{INK}{HTML}{595857}
\definecolor{YELLOW}{HTML}{f1c40f}
\definecolor{GREEN}{rgb}{0,0.6,0}
\definecolor{MIDGRAY}{rgb}{0.5,0.5,0.5}
\definecolor{MAUVE}{rgb}{0.58,0,0.82}

\usepackage{graphicx} 
\usepackage{libertine}


